ProsDectNet: Bridging the Gap in Prostate Cancer Detection via Transrectal B-mode Ultrasound Imaging

Interpreting traditional B-mode ultrasound images can be challenging due to image artifacts (e.g., shadowing, speckle), leading to low sensitivity and limited diagnostic accuracy. While Magnetic Resonance Imaging (MRI) has been proposed as a solution, it is expensive and not widely available. Furthermore, most biopsies are guided by Transrectal Ultrasound (TRUS) alone and can miss up to 52% cancers, highlighting the need for improved targeting. To address this issue, we propose ProsDectNet, a multi-task deep learning approach that localizes prostate cancer on B-mode ultrasound. Our model is pre-trained using radiologist-labeled data and fine-tuned using biopsy-confirmed labels. ProsDectNet includes a lesion detection and patch classification head, with uncertainty minimization using entropy to improve model performance and reduce false positive predictions. We trained and validated ProsDectNet using a cohort of 289 patients who underwent MRI-TRUS fusion targeted biopsy. We then tested our approach on a group of 41 patients and found that ProsDectNet outperformed the average expert clinician in detecting prostate cancer on B-mode ultrasound images, achieving a patient-level ROC-AUC of 82%, a sensitivity of 74%, and a specificity of 67%. Our results demonstrate that ProsDectNet has the potential to be used as a computer-aided diagnosis system to improve targeted biopsy and treatment planning.

==> images/_old_backup.tex <==
% Transrectal ultrasound (TRUS)-guided biopsy is a common method used to diagnose and plan treatment for prostate cancer. However, traditional B-mode ultrasound images can be difficult to interpret due to image artifacts such as speckle and shadowing, resulting in low sensitivity and limited diagnostic accuracy. Most studies have focused on using Magnetic Resonance Imaging (MRI) to address this issue, but it is expensive and not widely available. Moreover, 93\% of biopsies are guided by TRUS alone, and these biopsies miss up to 48\% cancers, thereby, it is important to improve the targeting of biopsies. Our study proposes a multi-task deep learning approach called ProsDectNet that localizes prostate cancer on B-mode ultrasound. Our model was pre-trained using radiologist-labeled data and fine-tuned using biopsy-confirmed labels. The model has a lesion detection and patch classification head, with uncertainty minimization using entropy to improve model performance and reduce false positive predictions. We trained and validated ProsDectNet using a cohort of 289 patients who underwent MRI-TRUS fusion targeted biopsy. We then tested our approach on a group of 41 patients and found that ProsDectNet achieves a patient-level ROC-AUC  of 82\%, a sensitivity of 74\%, and a specificity of 67\% outperforming average expert urologist in detecting prostate cancer on B-mode ultrasound images. ProsDectNet has the potential to be used as a computer-aided diagnosis system to improve targeted biopsy and treatment planning.

%One challenge with developing deep-learning methods for the analysis of B-mode ultrasound images is the lack of accurate labels. Manual annotation of B-mode ultrasound images without MRI and digital histology reports is a challenging and time-consuming task with high intra-variability. To reduce the cost of voxel-level annotation semi-supervised learning methods have been developed, including the mean-teacher framework \cite{Tarvainen2017}, co-training using pseudo-labels \cite{XIA2020101766,Qiao_2018_ECCV,pmlr-v172-luo22b}, and multi-planar training \cite{Zhou2019}, which have achieved good results in many semi-supervised medical image segmentation tasks. However, semi-supervised approaches may be sensitive if the labeled data is not representative of the entire distribution, which is particularly true in the case of B-mode ultrasound. B-mode TRUS images pose an additional challenge for detecting prostate cancer due to the similar appearance of cancerous tissue to other dark regions within the image. This similarity often leads to either over-segmentation of cancer regions or segment artifacts, which can result in false positive predictions by deep learning models 

% However, most of these studies have focused on classifying and grading prostate cancer based on the Gleason score, rather than localizing cancer. Detecting and spatially localizing prostate cancer on ultrasound images is crucial for targeted biopsy and treatment planning \cite{Azizi2018,Azizi2018b}.

% Fig. \ref{fig:flowchart} depicts our proposed multi-task framework (ProsDectNet) for localizing and detecting prostate cancer. The process begins by extracting random 3D patches $x \in \mathbf{R}^{h \times w \times z}$ from the prostate region, which are used to train the segmentation model $\mathcal{M}$ for supervised prostate cancer detection. $\mathcal{M}$ has an encoder with pyramid predictions at multiple scale for deep supervision. To minimize false positive predictions, the model incorporates two modules: (1) a classification head that uses the detection probability maps $\mathbf{P}_{x}$ of $\mathcal{M}$ to determine the presence or absence of cancer and (2) an uncertainty estimation head that computes the entropy map $\mathbf{E}_{x}$ from $\mathbf{P}_{x}$ and minimizes the entropy loss.

% \noindent\textbf{Patient-Level Evaluation.} Table \ref{tab:patient_level_eval} summarizes the patient-level evaluation results. ProsDectNet with pre-trained weights, classification head, and entropy loss achieved the best overall performance with a sensitivity of \textbf{74.0\%}, specificity of \textbf{67.0\%}, NPV of \textbf{74.0\%,} and accuracy of \textbf{70.0\%}. While the sensitivity was slightly lower compared to the ProsDectNet with classification head, the model was able to significantly improve specificity and reduce false positives rate from \textbf{23.0\%} $\rightarrow$ \textbf{67.0\%.} 



% \begin{table}[!t]
%     \centering
%     \caption{ Patient-level evaluations on test set. SE: sensitivity, SP: Specificity, PR: Precision, NPV: Negative predicted value, ACC: Accuracy. }
%     \label{tab:patient_level_eval}
%     \resizebox{0.60\textwidth}{!}{
%     \begin{tabular}{lccccc}
%     \hline
%     \textbf{Model} & \textbf{SE} & \textbf{SP} & \textbf{PR} & \textbf{NPV} & \textbf{ACC} \\
%     \hline
%     \textbf{3D-UNet \cite{3DUNet2016}} & x & x & x & x & x \\
%     \textbf{MT \cite{Tarvainen2017}} & x  & x & x& x & x  \\
%     \hline
%     \textbf{ProsDectNet} & 0.73 & 0.23 & 0.46 & 0.50 & 0.47 \\
%     + Pretrained + $\mathcal{L}_{Cls}$ & \textbf{0.79 }& 0.43 & 0.56 & 0.69 & 0.60 \\
%     + Pretrained + $\mathcal{L}_{Ent}$ & 0.74 & 0.57 & 0.61 & 0.71 & 0.65 \\
%     + Pretrained + $\mathcal{L}_{Cls}$ + $\mathcal{L}_{Ent}$ & 0.74 & \textbf{0.67} & \textbf{0.67} & \textbf{0.74} & \textbf{0.70} \\
%     \hline
%     \end{tabular}}
% \end{table}


% Adding the classification head not only improved the segmentation model's performance but also helped to penalize $\mathcal{M}$ and minimize false positive predictions specifically on normal B-mode TRUS images as compared to the baseline model.


% Entropy enables the exploration of structural consistency and reduces model uncertainty. For instance, B-mode TRUS images often exhibit different artifacts and lack clear boundaries between lesions and background tissue, which presents a challenge for detection models. Consequently, the model may either over-segment cancer regions or segment artifacts as lesions.
